CogALex-V Shared Task: LexNET - Integrated Path-based and Distributional Method for the Identification of Semantic Relations

We present a submission to the CogALex 2016 shared task on the corpus-based identification of semantic relations, using LexNET (Shwartz and Dagan, 2016), an integrated path-based and distributional method for semantic relation classification. The reported results in the shared task bring this submission to the third place on subtask 1 (word relatedness), and the first place on subtask 2 (semantic relation classification), demonstrating the utility of integrating the complementary path-based and distributional information sources in recognizing concrete semantic relations. Combined with a common similarity measure, LexNET performs fairly good on the word relatedness task (subtask 1). The relatively low performance of LexNET and all other systems on subtask 2, however, confirms the difficulty of the semantic relation classification task, and stresses the need to develop additional methods for this task.

==> images/confusion.tex <==
\setlength\tabcolsep{1.5pt}
\begin{tabular*}{\textwidth}{ccc}
\multicolumn{3}{c}{predictions} \\
\multirow{3}{*}{\rotatebox{90}{\centering gold}}

& \begin{tabularx}{.5\textwidth}{c|c|c|c|c|c|c|c|c|}
\hhline{~--------}
& sy & hy & ra & co & at & an & me & ev \\
\hhline{---------}
\multicolumn{1}{|c|}{syno} &  \cellcolor{brinkpink!1.123596}{1.12}  &  \cellcolor{brinkpink!57.303371}{57.30}  &  \cellcolor{brinkpink!3.745318}{3.75}  &  \cellcolor{brinkpink!1.872659}{1.87}  &  \cellcolor{brinkpink!2.247191}{2.25}  &  \cellcolor{brinkpink!12.734082}{12.73}  &  \cellcolor{brinkpink!10.112360}{10.11}  &  \cellcolor{brinkpink!10.861423}{10.86} \\
\hhline{---------}
\multicolumn{1}{|c|}{hyper} &  \cellcolor{brinkpink!0.049092}{0.05}  &  \cellcolor{brinkpink!56.701031}{56.70}  &  \cellcolor{brinkpink!24.447717}{24.45}  &  \cellcolor{brinkpink!4.074620}{4.07}  &  \cellcolor{brinkpink!1.374570}{1.37}  &  \cellcolor{brinkpink!2.700049}{2.70}  &  \cellcolor{brinkpink!5.792833}{5.79}  &  \cellcolor{brinkpink!4.860088}{4.86} \\
\hhline{---------}
\multicolumn{1}{|c|}{random} &  \cellcolor{brinkpink!0.149402}{0.15}  &  \cellcolor{brinkpink!5.079681}{5.08}  &  \cellcolor{brinkpink!78.585657}{78.59}  &  \cellcolor{brinkpink!0.747012}{0.75}  &  \cellcolor{brinkpink!2.788845}{2.79}  &  \cellcolor{brinkpink!1.145418}{1.15}  &  \cellcolor{brinkpink!4.083665}{4.08}  &  \cellcolor{brinkpink!7.420319}{7.42} \\
\hhline{---------}
\multicolumn{1}{|c|}{cohyp} &  \cellcolor{brinkpink!0.000000}{0.00}  &  \cellcolor{brinkpink!3.884462}{3.88}  &  \cellcolor{brinkpink!66.384462}{66.38}  &  \cellcolor{brinkpink!26.494024}{26.49}  &  \cellcolor{brinkpink!0.398406}{0.40}  &  \cellcolor{brinkpink!0.597610}{0.60}  &  \cellcolor{brinkpink!1.593625}{1.59}  &  \cellcolor{brinkpink!0.647410}{0.65} \\
\hhline{---------}
\multicolumn{1}{|c|}{attri} &  \cellcolor{brinkpink!0.000000}{0.00}  &  \cellcolor{brinkpink!3.886555}{3.89}  &  \cellcolor{brinkpink!10.084034}{10.08}  &  \cellcolor{brinkpink!0.945378}{0.95}  &  \cellcolor{brinkpink!76.365546}{76.37}  &  \cellcolor{brinkpink!2.205882}{2.21}  &  \cellcolor{brinkpink!2.626050}{2.63}  &  \cellcolor{brinkpink!3.886555}{3.89} \\
\hhline{---------}
\multicolumn{1}{|c|}{anto} &  \cellcolor{brinkpink!0.501253}{0.50}  &  \cellcolor{brinkpink!32.832080}{32.83}  &  \cellcolor{brinkpink!6.265664}{6.27}  &  \cellcolor{brinkpink!8.270677}{8.27}  &  \cellcolor{brinkpink!12.531328}{12.53}  &  \cellcolor{brinkpink!28.070175}{28.07}  &  \cellcolor{brinkpink!5.263158}{5.26}  &  \cellcolor{brinkpink!6.265664}{6.27} \\
\hhline{---------}
\multicolumn{1}{|c|}{mero} &  \cellcolor{brinkpink!0.410509}{0.41}  &  \cellcolor{brinkpink!10.016420}{10.02}  &  \cellcolor{brinkpink!18.390805}{18.39}  &  \cellcolor{brinkpink!2.791461}{2.79}  &  \cellcolor{brinkpink!1.477833}{1.48}  &  \cellcolor{brinkpink!0.574713}{0.57}  &  \cellcolor{brinkpink!60.509031}{60.51}  &  \cellcolor{brinkpink!5.829228}{5.83} \\
\hhline{---------}
\multicolumn{1}{|c|}{event} &  \cellcolor{brinkpink!0.000000}{0.00}  &  \cellcolor{brinkpink!3.838174}{3.84}  &  \cellcolor{brinkpink!2.697095}{2.70}  &  \cellcolor{brinkpink!0.311203}{0.31}  &  \cellcolor{brinkpink!0.726141}{0.73}  &  \cellcolor{brinkpink!0.207469}{0.21}  &  \cellcolor{brinkpink!5.394191}{5.39}  &  \cellcolor{brinkpink!86.825726}{86.83} \\
\hhline{---------}
\end{tabularx}

& \begin{tabularx}{.5\textwidth}{c|c|c|c|c|c|c|c|c|}
\hhline{~--------}
& sy & hy & ra & co & at & an & me & ev \\
\hhline{---------}
\multicolumn{1}{|c|}{syno} &  \cellcolor{brinkpink!28.464419}{28.46}  &  \cellcolor{brinkpink!28.838951}{28.84}  &  \cellcolor{brinkpink!4.119850}{4.12}  &  \cellcolor{brinkpink!1.872659}{1.87}  &  \cellcolor{brinkpink!3.745318}{3.75}  &  \cellcolor{brinkpink!22.097378}{22.10}  &  \cellcolor{brinkpink!9.737828}{9.74}  &  \cellcolor{brinkpink!1.123596}{1.12} \\
\hhline{---------}
\multicolumn{1}{|c|}{hyper} &  \cellcolor{brinkpink!3.583702}{3.58}  &  \cellcolor{brinkpink!80.657830}{80.66}  &  \cellcolor{brinkpink!4.663721}{4.66}  &  \cellcolor{brinkpink!2.209131}{2.21}  &  \cellcolor{brinkpink!1.521846}{1.52}  &  \cellcolor{brinkpink!2.896416}{2.90}  &  \cellcolor{brinkpink!2.896416}{2.90}  &  \cellcolor{brinkpink!1.570938}{1.57} \\
\hhline{---------}
\multicolumn{1}{|c|}{random} &  \cellcolor{brinkpink!0.348606}{0.35}  &  \cellcolor{brinkpink!7.171315}{7.17}  &  \cellcolor{brinkpink!79.033865}{79.03}  &  \cellcolor{brinkpink!2.340637}{2.34}  &  \cellcolor{brinkpink!1.095618}{1.10}  &  \cellcolor{brinkpink!0.448207}{0.45}  &  \cellcolor{brinkpink!4.780876}{4.78}  &  \cellcolor{brinkpink!4.780876}{4.78} \\
\hhline{---------}
\multicolumn{1}{|c|}{cohyp} &  \cellcolor{brinkpink!0.000000}{0.00}  &  \cellcolor{brinkpink!1.045817}{1.05}  &  \cellcolor{brinkpink!1.245020}{1.25}  &  \cellcolor{brinkpink!95.866534}{95.87}  &  \cellcolor{brinkpink!0.149402}{0.15}  &  \cellcolor{brinkpink!0.099602}{0.10}  &  \cellcolor{brinkpink!1.145418}{1.15}  &  \cellcolor{brinkpink!0.448207}{0.45} \\
\hhline{---------}
\multicolumn{1}{|c|}{attri} &  \cellcolor{brinkpink!1.155462}{1.16}  &  \cellcolor{brinkpink!2.941176}{2.94}  &  \cellcolor{brinkpink!1.785714}{1.79}  &  \cellcolor{brinkpink!0.420168}{0.42}  &  \cellcolor{brinkpink!86.554622}{86.55}  &  \cellcolor{brinkpink!4.411765}{4.41}  &  \cellcolor{brinkpink!1.575630}{1.58}  &  \cellcolor{brinkpink!1.155462}{1.16} \\
\hhline{---------}
\multicolumn{1}{|c|}{anto} &  \cellcolor{brinkpink!12.280702}{12.28}  &  \cellcolor{brinkpink!15.538847}{15.54}  &  \cellcolor{brinkpink!2.005013}{2.01}  &  \cellcolor{brinkpink!0.751880}{0.75}  &  \cellcolor{brinkpink!9.273183}{9.27}  &  \cellcolor{brinkpink!50.877193}{50.88}  &  \cellcolor{brinkpink!8.521303}{8.52}  &  \cellcolor{brinkpink!0.751880}{0.75} \\
\hhline{---------}
\multicolumn{1}{|c|}{mero} &  \cellcolor{brinkpink!1.395731}{1.40}  &  \cellcolor{brinkpink!5.008210}{5.01}  &  \cellcolor{brinkpink!4.844007}{4.84}  &  \cellcolor{brinkpink!1.888342}{1.89}  &  \cellcolor{brinkpink!0.574713}{0.57}  &  \cellcolor{brinkpink!1.806240}{1.81}  &  \cellcolor{brinkpink!82.183908}{82.18}  &  \cellcolor{brinkpink!2.298851}{2.30} \\
\hhline{---------}
\multicolumn{1}{|c|}{event} &  \cellcolor{brinkpink!0.000000}{0.00}  &  \cellcolor{brinkpink!1.141079}{1.14}  &  \cellcolor{brinkpink!3.319502}{3.32}  &  \cellcolor{brinkpink!0.414938}{0.41}  &  \cellcolor{brinkpink!0.518672}{0.52}  &  \cellcolor{brinkpink!0.103734}{0.10}  &  \cellcolor{brinkpink!1.659751}{1.66}  &  \cellcolor{brinkpink!92.842324}{92.84} \\
\hhline{---------}
\end{tabularx}
\\
& \textbf{Path-based} & \textbf{Distributional}
\end{tabular*}
